Taming Subgraph Isomorphism for RDF Query Processing

RDF data are used to model knowledge in various areas such as life sciences, Semantic Web, bioinformatics, and social graphs. The size of real RDF data reaches billions of triples. This calls for a framework for efficiently processing RDF data. The core function of processing RDF data is subgraph pattern matching. There have been two completely different directions for supporting efficient subgraph pattern matching. One direction is to develop specialized RDF query processing engines exploiting the properties of RDF data for the last decade, while the other direction is to develop efficient subgraph isomorphism algorithms for general, labeled graphs for over 30 years. Although both directions have a similar goal (i.e., finding subgraphs in data graphs for a given query graph), they have been independently researched without clear reason. We argue that a subgraph isomorphism algorithm can be easily modified to handle the graph homomorphism, which is the RDF pattern matching semantics, by just removing the injectivity constraint. In this paper, based on the state-of-the-art subgraph isomorphism algorithm, we propose an in-memory solution, TurboHOM++, which is tamed for the RDF processing, and we compare it with the representative RDF processing engines for several RDF benchmarks in a server machine where billions of triples can be loaded in memory. In order to speed up TurboHOM++, we also provide a simple yet effective transformation and a series of optimization techniques. Extensive experiments using several RDF benchmarks show that TurboHOM++ consistently and significantly outperforms the representative RDF engines. Specifically, TurboHOM++ outperforms its competitors by up to five orders of magnitude.

==> optimization.tex <==
\section{Optimization}
\label{sec:optimization}

In this section, we introduce four optimizations that we apply on \TurboISOp{}
to improve its efficiency of RDF query processing.  These optimizations are
created by observing the characteristics of RDF data and are therefore specific to
RDF data. Even though these optimizations do not change \TurboISOp{} severely,
they could improve the query processing efficiency quite significantly.

% \begin{figure*}[t]
%   \begin{tabular}{c}
%   \subfloat[t][query tree of Figure~\ref{fig:type-ware-trans-query-q2}.]
%   {
%     \label{fig:nec-q2}
%     \hspace{1cm}
%     \includegraphics[width=0.18\linewidth]{nec-q2}
%     \hspace{1cm}
%   }
%   \\
%   \subfloat[t][candidate region.]
%   {
%     \label{fig:cr-q2}
%     \includegraphics[width=0.32\linewidth]{cr-q2}
%   }
%   \end{tabular}
%   \begin{tabular}{c}
%   \subfloat[t][data vertex binding first.]
%   {
%     \label{fig:bind-first}
%     \raisebox{0.6cm}{\includegraphics[width=0.3\linewidth]{bind-first}}
%   }
%   \\
%   \subfloat[non-tree edge test next.]
%   {
%     \label{fig:check-next}
%     \includegraphics[width=0.3\linewidth]{check-next}
%   }
%   \end{tabular}
%   \begin{tabular}{c}
%   \subfloat[non-tree edge test first.]
%   {
%     \label{fig:check-first}
%     \includegraphics[width=0.32\linewidth]{check-first}
%   }
%   \\
%   \subfloat[data vertex binding next.]
%   {
%     \label{fig:bind-next}
%     \includegraphics[width=0.3\linewidth]{bind-next}
%   }
%   \end{tabular}
%   \caption{Example of non-tree matching using intersection (matching
%     order: $u_1 \to u_2 \to u_0$, shaded vertex: bound vertex,
%     (c)--(d): original implementation, (e)--(f) modified
%     implementation).}
%   \label{fig:non-tree-merge}
% \end{figure*}


\paragraph*{Use intersection on $IsJoinable$ test \textsf{(+INT)}}
\label{sec:non-tree-edge}

\edit{\sloppy We optimize the $IsJoinable$ test in $SearchSubgraph$.
$SubgraphSearch$ checks the $IsJoinable$ test by repetitive calls to
the membership operation. However, the optimization allows a bulk of
$IsJoinable$ tests with one intersection operation.}

\edit{$SearchSubgraph$ checks the existence of the edges between the current
candidate data vertex and the already bounded data vertices by calling
$IsJoinable$ (line 7 of Algorithm~\ref{alg:subgraphsearch}. Let us
consider the query graph (Figure~\ref{fig:type-ware-trans-query-q2})
and a data graph (Figure~\ref{fig:opt-intersection}). Suppose that,
for a given matching order $u_1 \to u_2 \to u_0$, the vertex $v_1$ is
bound to $u_1$, and the vertex $v_2$ is bound to $u_2$. Then, the next
step it to bind a data vertex to $u_0$. Because there is an edge
between $u_0$ and $u_2$, to bind a data vertex of ID $v_i (i
=0,3,4,\cdots,1001$) to $u_o$, we need to check whether there exists
an edge $v_i \to v_2$.}

\begin{figure}[h!]
  \centering
  \label{fig:data-graph}
  \includegraphics[width=0.8\linewidth]{data-graph}
  \caption{An example data graph for illustrating \textsf{+INT}.}
  \label{fig:opt-intersection}
\end{figure}

\edit{$IsJoinable$ checks for the existence of the edge between the current
data vertex and already matched data vertices by repetitively calling
$IsJoinable$. Let us consider the above example. For each $v_i (i =
0,3,4,\cdots,1001)$, $IsJoinable$ tests whether the edge $v_i \to v_2$
exists. If $v_2$ is a member of $v_i$'s outgoing adjacency list, the
test succeeds and the graph matching continues.}

\edit{Instead, our modified $IsJoinable$ tests all the edge existences
  between the current candidate vertices ($C_{R}$ in line 5 of
  Algorithm~\ref{alg:subgraphsearch}) and the already matched data
  vertices by one intersection operation. Let us consider the above
  example again. The modified $IsJoinable$ finds the edge between
  $v_2$ and the candidate data vertices $v_0,v_3,\cdots,v_{1001}$ at
  once. For this, it is enough to perform one intersection operation
  between the $v_2$'s incoming adjacency vertices and the candidate
  data vertices. Since the modified $IsJoinable$ takes $C_R$ as a
  parameter, the line 6 and 7 of Algorithm~\ref{alg:subgraphsearch} are
  merged into one statement.}

\edit{Note that this optimization can improve the performance
  significantly. In the above example, since only $v_0$ and $v_{1001}$
  pass the test, we can skip calling the original $IsJoinable$ $998$
  times. Formally speaking, suppose that the degree of the already
  matched data vertex, $v_{matched}$, is $deg(v_{matched})$ and the
  number of candidate data vertices is $|C_{R}|$ (line 6 of
  Algorithm~\ref{alg:subgraphsearch})\footnote{As a reminder, the
    ``such that v is not yet matched'' constraint does not apply in
    the graph homomorphism (See Section~\ref{sec:gener-subgr-isom}).}.
  The complexity of the original $IsJoinable$ test is $O(|C_{R}|\log
  deg(v_{matched})$ in that $IsJoinable$ is called $|C_{R}|$ time and
  $O(\log deg(v_{matched}))$ is required when conducting a binary
  search of a specified neighbor among $deg(v_{matched})$ neighbors.
  On the contrary, the complexity of the modified $IsJoinable$ test is
  $\min(|C_{R}| + deg(v_{matched}),$ $|C_{R}| \log deg(v_{matched}))$
  since the modified $IsJoinable$ can choose the intersection strategy
  among merging and binary searches based on the $deg(v_{matched})$
  size. }



%--------- THIS paragraph is about homomorphism -----------------------------
% \paragraph*{Disable Data Vertex Bound Test \textsf{(-BOUND)}}
% \label{sec:disable-bound-vertex}

% In the original \TurboISO{}, the embedding is assumed to be a one-to-one
% function. In other words, once a data vertex is bound to a query vertex, it is
% not allowed to be bound to any other query vertices in the same embedding. For
% example, the embedding in Figure~\ref{fig:disable-visit-vertex-test} is not a
% valid embedding in subgraph isomorphism. The one-to-one mapping in subgraph
% isomorphism ensures that the enumerated subgraph has the same topology as the
% query graph. To enforce the one-to-one mapping, the original \TurboISO{}
% maintains the visited vertex set, and rejects the current embedding when it
% tries to map an already bound data vertex to a query vertex.

% However, for RDF query processing, the embedding is a one-to-many function.
% That means a data vertex can be bound to multiple query vertices. So, in RDF
% query processing, the embedding of Figure~\ref{fig:disable-visit-vertex-test}
% is a valid embedding~\footnote{Note that this matching semantic is not defined
% by SPARQL specification but agreed upon by RDF engine implementations. Commercial RDF engines follow this matching semantics.}  Accordingly, our modified \TurboISO{} neither stores the
% bound vertices in the current embedding, nor tests whether a data vertex has
% already been bound to a query vertex in $SearchSubgraph$ (line 7 of
% Algorithm~\ref{alg:turboiso}).

% \begin{myverbbox}{\vonetomany}
%   SELECT ?a, ?b1, ?b2 WHERE
%   { ?a rdf:type X. ?b1 rdf:type Y. ?b2 rdf:type Y.
%     ?a x ?b1; x ?b2. }
% \end{myverbbox}

% \begin{figure}[h!]
%   \centering
%   \begin{verbatim}
%   SELECT ?a, ?b1, ?b2 WHERE
%   { ?a rdf:type X. ?b1 rdf:type Y. ?b2 rdf:type Y.
%     ?a x ?b1; x ?b2. }
%     \end{verbatim}
%   \includegraphics[width=0.7\linewidth]{disable-visit-vertex-check}
%   \caption{One-to-many vertex embedding (in subgraph isomorphism: no,
%     in SPARQL: yes).}
%   \label{fig:disable-visit-vertex-test}
% \end{figure}

\paragraph*{Reuse Matching Order (\textsf{+REUSE})}
\label{sec:reuse-matching-order}

The second optimization is to reuse the matching order of the first
candidate region for all the other candidate regions. \edit{Note that
  this optimization is specific to \TurboISOp{}.}
% That is, \linebreak $DetermineMatchingOrder$ (line 6 of
% Algorithm~\ref{alg:turboiso}) is called only once throughout the
% \TurboISO{} execution, and the same matching order is used throughout
% the query processing.
\TurboISOp{} used a different matching order different matching order
for each candidate region, because each candidate region could have a
very different number of candidate vertices for a given query path in
\edit{graph homomorphism} problems. However, typical RDF datasets are
regular at the schema level, and generating the
matching order for each candidate regions is ineffective, especially
when the size of each candidate region is small. We also performed
experiments with more irregular, heterogeneous datasets, including
YAGO and BTC2012. This optimization technique did not incur suboptimal
matching performance as we will see in our extensive experiments in
Section~\ref{sec:experiment}..

% inefficient.

Let us take the example of the expanded RDF data from
Figure~\ref{fig:rdf} and the query graph of
Figure~\ref{fig:type-ware-trans-query-q2}. Suppose that the query tree
is Figure~\ref{fig:nec-q2}. In that case, the starting data vertices
of the candidate regions are the data vertices with the
\verb|University| vertex label. To make a candidate region for a
starting data vertex, \verb|univ1|, we must find (1) all departments
in \verb|univ1| and (2) all the graduate students who got their
undergraduate degrees from \verb|univ1|. Because the selectivity of
(2) is higher than that of (1), the matching order, $u_1 \to u_2 \to
u_0$ is chosen. For the other universities (starting vertices), it is
rare that the selectivity of (2) is higher than that of (1). For such
a case, it is more efficient to reuse the first matching order.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.35\linewidth]{nec-q2}
  \caption{A query tree of the query graph of
    Figure~\ref{fig:type-ware-trans-query-q2}.}
  \label{fig:nec-q2}
\end{figure}

\paragraph*{Disable Degree Filter \textsf{(-DEG)}}
\label{sec:disable-degr-filt}

\edit{The third optimization is to disable the degree filter. The
  degree filter might be effective when the degrees of data vertices
  having the same vertex label are irregular. However, since the
  degree distribution is regular in RDF datasets, the degree filter is
  not helpful for such regular distributions. This optimization is
  applicable to all \edit{graph homormorphism} algorithm that uses
  degree filter such as \TurboISO{} \cite{HLL:13aa} and Ullman
  \cite{U:76aa}. }

% The third optimization is to disable the degree filter in
% $ExploreCandidateRegion$ (line 4 of Algorithm~\ref{alg:turboiso}). The
% degree filter is used by the original \TurboISO~\cite{HLL:13aa}, which
% prunes out depth-first search on the data vertex that has a lower
% degree than its corresponding query vertex. Although the degree filter
% might be effective when the degrees of data vertices having the same
% vertex label are irregular, the degree distribution is regular in RDF
% datasets. Since the degree filter is not helpful for such regular
% distributions, we disable it in our modified \TurboISO{}.

\paragraph*{Disable NLF Filter \textsf{(-NLF)}}
\label{sec:disable-nlf-filter}

\edit{The last optimization is to disable the NLF filter. Similar to
  the degree filter, the NLF filter is effective when the degree and
  the neighbor types are very irregular while RDF datasets typically
  are not. This optimization is applicable to all graph homormorphism
  algorithm that uses the NLF filter such as \TurboISO{}
  \cite{HLL:13aa} and GraphQL \cite{HS:08aa}.}

% The last optimization is to disable the NLF filter in
% $ExploreCandidateRegion$ (line 4 of Algorithm~\ref{alg:turboiso}).
% After the degree filter is passed, the original \TurboISO{} tests
% whether the current explored data vertex has a high enough number of
% neighbors for all neighbor types in the corresponding query vertex.
% Similar to the degree filter, the NLF filter is effective when the
% degree and the neighbor types are very irregular while RDF datasets
% typically are not. So, the modified \TurboISO{} again disables the NLF
% filter.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "turbordf.pvldb"
%%% End:


==> queries.tex <==
% \section{Queries}
% \label{sec:queries}

% \subsection{LUBM}
% \label{sec:lubm}
% \scriptsize
% \noindent PREFIX rdf: <http://www.w3.org/1999/02/22-rdf-syntax-ns\#> \\
% PREFIX ub: <http://www.lehigh.edu/~zhp2/2004/0401/univ-bench.owl\#>

% \textbf{Q1.}
% SELECT ?X	
% WHERE
% {?X rdf:type ub:GraduateStudent . \\
%   ?X ub:takesCourse
% <http://www.Department0.University0.edu/GraduateCourse0>}


% \subsection{BSBM}
% \label{sec:bsbm}

% \subsection{Yago}
% \label{sec:yago}

% \subsection{DBPedia}
% \label{sec:dbpedia}

% \subsection{BTC 2012}
% \label{sec:btc-2012}



%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "turbordf.sigmod2015"
%%% End: 


==> revision-note.tex <==
\newpage
\normalsize
{\Large \bfseries \noindent Summary of Revision \\}

\noindent Dear reviewers,\\

We deeply appreciate your careful comments. We hope the revised
version addresses all reviewers' questions and clarification requests. The
comments of the reviewers were very helpful in improving the quality
of the paper. We detail our responses below.\\

{\large \bfseries \noindent Specific revisions requested by reviewers \\}

\noindent \textbf{\large Reviewer 1 \\}

\noindent The first reviewer (R1) asked us to respond to specific revisions for D1 -- D5. \\


\noindent \textbf{{R1.D1-1. When the authors state the ``important research
	problem'', is it the graph exploration alone or the combination graph
		exploration and IsJoinable? Please clarify.
} \\}

The research problem we solve in this paper is ``Can subgraph isomorphism
be tamed for efficient RDF processing?'' According to our profiling
results in our response to R1.W1, there exist two major subtasks in
\TurboISO{}, 1) exploring candidate subgraphs in $ExploreCandidateRegion$
and 2) enumerating solutions based on candidate regions in $SubgraphSearch$.
Thus, the problem involves both efficient graph exploration and tailored
optimization techniques including +INT. \TurboISOP{} is the first system
to solve this important problem. In order to clarify our problem, we
have revised the first paragraph in page 2 as follows: \\

\textit{
``Is this phenomenon due to inherent limitations of the graph homomorphism (subgraph isomorphism) algorithm?''
  Our profile results show that two major subtasks
  of \TurboISO{} --- 1) exploring candidate subgraphs in $ExploreCandidateRegion$ and 2)
  enumerating solutions based on candidate regions in $SubgraphSearch$ --- require performance improvement. \TurboISOP{} resolves such performance hurdles by
  proposing the type-aware transformation and tailored
  optimization techniques. \\
  }

\noindent \textbf{{R1.D1-2. In addition, how much time is needed to finish the numerous IsJoinable tests.} \\}

Please refer to the response to R1.W1. \\

\noindent \textbf{{R1.D1-3. Can the paper and its experiment provide more evidences to illustrate the main research problem and they are solved by any specific proposed techniques?
} \\}

Our profiling results showed that there exist two major performance bottlenecks in
\TurboISOp{}, and we proposed type-aware transformation for the first
bottleneck and a series of tailored optimization techniques for both
bottlenecks. We also analyzed the effect of type-aware transformation and
each optimization technique in our experiments. Thus, we have revised our
paper accordingly. Thank you very much for your valuable comment. \\

\noindent \textbf{{R1.D2. RDF-3X and TripleBit were built on top of
  MonetDB. Their systems and experiments did not expect all data to be
  loaded into the main memory. It may be more fair to run TurboHOM on
  a machine that are similar to those were used in RDF-3X or
  TripleBit, e.g. 64G memory. This will clarify if the performance
  gain is due to a nice main-memory graph representation, i.e., not
  just because of the algorithms/optimization ideas presented in the
  paper. If the proposed technique was main-memory, please clearly
  states so. If no, please add an experiment to show how the systems
  behave as the available memory varies.}\\}

As per request, we have stated more clearly in the abstract and Section~\ref{sec:introduction} that \TurboISOP{} 1) is
main-memory based and 2) aims to serve
as an RDF processing accelerator on top of the Oracle RDBMS. \\

In abstract: \\
\textit{$\dots$ In this paper, based on the state-of-the-art subgraph
  isomorphism algorithm, we propose an in-memory solution,
  \TurboISOP{}, which is tamed for the RDF processing $\dots$}

In Section~\ref{sec:introduction}: \\
\textit{In this paper, based on the state-of-the-art subgraph
  isomorphism algorithm \cite{HLL:13aa}, we propose an in-memory
  solution, \TurboISOP{}, which is \edit{tamed} for the RDF
  processing, $\cdots$ Our method aims to serve as an RDF
  accelerator on top of the Oracle RDBMS. \\ }

RDF-3X and TripleBit have considered both cold and warm run conditions
and have presented their performance under both conditions. When a machine
has enough memory, a whole RDF dataset is resident in main memory during hot runs. In
such a case, their hot run performance is in the same ballpark as
the performance of main-memory solutions. In addition, TripleBit did compare its
performance with a main-memory solution, BitMat, and claimed its superiority when a whole dataset
is resident in main-memory. Note that both systems are not on top of MonetDB, which was confirmed by the original authors and their source code.

 Note that the performance gain is mainly due to the algorithms/optimization techniques presented. Unlike existing RDF processing engines, which rely
 on joins, the proposed systems are based on graph exploration algorithms,
 which show good performance when queries require a small amount of graph
 exploration. In order to optimize queries requiring a large amount of graph
 exploration, we propose the type-aware transformation as well as a series
 of optimization techniques. We also analyze the effect of each improvement
 technique in Section~\ref{sec:effect-optimization}.
\\

\noindent \textbf{{R1.D3. Type-aware transformation is one of the main techniques of the paper. However, its description is causal. For example, in the last paragraph of Section 4.1, ``t vertices ... in q are *embedded* as vertex labels in q'. Then, no data vertices ... exist under the type-aware transformation.'' Section 4.1 should be formalized.} \\}

Section 4.1 has been significantly revised by formally defining the type-aware transformation
(see Definition~\ref{def:type-aware} below).

\setcounter{definition}{2}

\begin{definition}
  \label{def:type-aware}
  The type-aware transformation $(F_V, F_{ID}, F_E,$ $F_{VL},F_{EL})$
  converts a set of triples $T(S, P, O)$ to a type-aware transformed
  graph $G(V,E,ID,L)$.  Let us divide $T$ into three disjoint subsets
  whose union is $T$ --- $T'(S',P',O')$,
  $T'_{\mathsf{t}}(S'_{\mathsf{t}}, P'_{\mathsf{t}}, O'_{\mathsf{t}})
  = \{(s,\text{rdf:type},o) \in T\}$,
  and
  $T'_{\mathsf{sc}}(S'_{\mathsf{sc}}, P'_{\mathsf{sc}},
  O'_{\mathsf{sc}}) = \{(s,\text{rdf:subClassOf},o) \in T \}$.

  \begin{enumerate}[1.,leftmargin=0.4cm]
    \setlength{\itemsep}{-3pt}
  \item A vertex mapping $F_V: S' \cup O' \cup S'_\mathsf{t} \to V$,
    which is bijective, maps a subject in $S' \cup S'_\mathsf{t}$ or
    an object in $O'$ to a vertex.
  \item A vertex ID mapping
    $F_{ID}: S' \cup O' \cup S'_\mathsf{t} \to N \cup \{\_\}$, which
    is bijective, maps a subject in $S' \cup S'_\mathsf{t}$ or an
    object in $O'$ to a vertex ID or blank. Here, $F_{ID}(x) = \_$ if x
    is a variable.
  \item An edge mapping $F_E: T' \to E$, which is bijective, maps a
    triple of $T'$ into an edge, $F_E(s,p,o) = (F_V(s), F_V(o))$.
  \item A vertex label mapping
    $F_{VL} : O'_\mathsf{t} \cup O'_{\mathsf{sc}} \to VL \cup \{\_\}$, which is
    bijective, maps an object of $O'_\mathsf{t} \cup O'_{\mathsf{sc}}$
    into a vertex label. Here, $F_{VL}(x) = \_$ if x is a variable.
  \item An edge label mapping $F_{EL} : P' \to EL \cup \{\_\}$, which is
    bijective, maps a predicate of $P'$ into an edge label. Here, $F_{EL}(x) = \_$ if x is a variable.
  \item A vertex ID mapping function $ID: V \to N$ maps a
    vertex to a vertex ID where
    $ID(v) = F_{ID} \circ F_V^{-1}(v)$.
  \item A labeling function $L$ 1) maps a vertex to a set of vertex labels such that $v \in V$,
    $L(v) = \{F_{VL}(o) | \text{ there is a path from }$ $F_V^{-1}(v)
	\text{ to } o \text{ using triples in } T'_{\mathsf{t}} \cup T'_{\mathsf{sc}}\}$ and 2) maps an edge e to an edge label such that $e \in E$, $L(e) = F_{L_E}(Pred(F_E^{-1}(e)))$ where
	$Pred(s,p,o) = p$.
  \end{enumerate}
  \vspace{-1mm}
\end{definition}

\vspace{-2mm}
\noindent \textbf{R1.D4. It was argued that RDF graphs are regular in practice. But, in Section 6, a simple assignment of start vertex ``may lead to load imbalance''. Please further elaborate what are causes the imbalance.}

\noindent \textbf{=R1.W2. There are some contradicting observations when the authors motivate some optimizations. For example, when the authors present +REUSE, they argue that the ``RDF datasets do not have such extremely irregular candidate regions''. These observations motivate -DEG and -NLF as well. In comparison, when the authors motivate parallel processing, the authors argue ``the actual amount of graph exploration varies can be different for each starting data vertex''. Let's assume both arguments were true at the same time. Then, the authors may further convince readers how similar candidate regions lead to different graph explorations, to what degree and how common they are, in practice. \\}

   We meant that typical RDF data sets are regular at the \textit{schema} level, i.e.,
  well-structured in practice~\cite{NM:11aa,GN:14aa}. Although RDF datasets are
  regular at the schema-level, the cardinalities of one (many)-to-many
  relationships can significantly vary in candidate regions. This property
  even holds for joins in relational databases. For example in
  Figure~\ref{fig:type-ware-trans-query-q2}, the query involves three
  types, university, graduate students, and departments at the schema level
  while universities can have significantly different numbers of
  graduated students and departments.
   We performed experiments with more irregular, heterogeneous datasets,
   including YAGO and BTC2012. These optimization techniques do not
   incur suboptimal matching performance.\\

  %In the paper, the meaning of `regular' was not clearly stated. We
%stated that degree and neighbor type distribution is `regular' in the
%schema level~\cite{NM:11aa,GN:14aa}. Thus, the matching order
%is same for all candidate regions. However, in the instance level, the
%cardinality of a one(many)-to-many relation varies on each data
%vertex, which also holds joins in relational databases. Such
%irregularity in the instance level induces workload imbalance when
%parallelizing. \\

We elaborated the description of regularity of RDF datasets in
Section~\ref{sec:disable-degr-filt} as follows. \\

\textit{The second optimization is to disable the NLF filter in
$ExploreCandidateRegion$. The NLF filter may be effective when the
neighbor type are very irregular. However, in practice, most RDF datasets
are structured~\cite{NM:11aa,GN:14aa}. For example, in our sample RDF
dataset (Figure~\ref{fig:graph}), in most cases, a vertex corresponding
to a graduate student has} \verb|telephone|, \verb|emailAddress|,
\verb|memberOf|, and \verb|undergraduateDegreeFrom|
\textit{predicates. Accordingly, the NLF filter is not helpful for such
  structured RDF datasets. \\}

\textit{The third optimization is to disable the degree filter in
  $ExploreCandidateRegion$. Similar to the NLF filter, the degree
  filter is effective when the degree is very irregular while RDF
  datasets typically are not. \\}

  \textit{ ...
However, typical RDF datasets are regular
at the schema level, i.e. well structured in practice, and generating the
matching order for each candidate regions is ineffective, especially
when the size of each candidate region is small. We also performed
experiments with more heterogeneous datasets, including Yet
Another Great Ontology (YAGO) \cite{SKW:08aa}, and Billion Triples Challenge 2012 (BTC2012) \cite{H:12aa}.
This optimization technique still shows good matching performance as we will see in our extensive experiments in Section~\ref{sec:experiment}, since these heterogeneous datasets do not show extreme irregularity at the schema level.\\}

We elaborated the description of the workload
imbalance in Section~\ref{sec:parallel-processing} as follows. \\

\textit{However, distributing the starting data vertices in a
  pre-determined way may lead to workload imbalance on threads. Although RDF datasets are
  regular at the schema-level, the cardinalities of one (many)-to-many
  relationships at the instance-level can significantly vary in candidate regions. This property
  even holds for joins in relational databases. For example, in
  Figure~\ref{fig:type-ware-trans-query-q2}, the query involves three
  types, University, Graduate students, and Departments at the schema level
  while universities can have significantly different numbers of
  graduated students and departments, which leads to different workload for each
  university vertex. To have as even a workload for each thread as
  much as possible, we assign a small chunk of the starting data
  vertices to threads dynamically. \\}

\noindent \textbf{{R1.D5. Section 5 lacks technical depth, where trivial and/or classic techniques are adopted (with minor modifications). Please highlight if there is anything new in this section.} }

\noindent \textbf{{=R1.W3. There are no non-trivial/novel techniques for the support of general SPARQL keywords. A similar comment applies to the section on parallel processing.} \\}

Note that OPTIONAL clauses can be handled by classical left outer join, although both RDF-3X and TripleBit do not support this functionality. However,
\TurboISOP{} is based on graph exploration rather than join. Specifically, it handles
OPTIONAL keywords both in $ExploreCandidateRegion$ and $SubgraphSearch$.
Thus, we present a simple yet effective technique for \TurboISOP{} based on two strategies,
\textit{nullify-and-keep-searching}, and \textit{qualify-and-exclude-duplicate}. We have revised Section~\ref{sec:pattern-modifier} as follows. \\

\textit{ To support queries that ask information which is not
  necessarily required, the OPTIONAL keyword is
  used. Figure~\ref{fig:optional} is an example of such a query which
  finds the price of} \verb|<product1>| \textit{and its rating and its
  homepages if possible. To handle OPTIONAL in \TurboISOP{}, we propose a
  simple yet effective technique as follows. First, \TurboISOP{}
  selects a start query vertex which is not specified in an OPTIONAL
	  clause. Then,
  \TurboISOP{} makes a candidate solution using the
  \emph{nullify-and-keep-searching} strategy. In
  $ExploreCandidateRegion$, if the current query vertex is in an OPTIONAL clause,
  and no data vertex is matched, \TurboISOP{} nullifies the current
  query vertex mapping in a candidate region. In $SubgraphSearch$,
  even though the mapped data vertex is nullified, if the
  corresponding query vertex is in an OPTIONAL clause, it invokes a recursive
  call. After a candidate solution is constructed using
  nullify-and-keep-searching, \TurboISOP{} qualifies it using the
  \emph{qualify-and-exclude-duplicate} strategy. The OPTIONAL semantics
  enforces that all vertices in an OPTIONAL clause must be mapped to data vertices,
  otherwise, the mappings of all query vertices in an OPTIONAL clause are
  nullified. Also, when all vertices in an OPTIONAL clause are nullified, the
  nullified final mapping should be generated only once. \TurboISOP{}
  excludes the duplicates by comparing the current final mapping with
  the previous valid mapping. For example, suppose two successive
  solutions of the example query are}
$\{$\verb|(price,$100)|, \verb|(rating, 5)|,
\verb|(homepage,null)|$\}$,
\textit{and} $\{$\verb|(price,$100)|,
\verb|(rating, 1)|, \verb|(homepage,null)|$\}$. \textit{The preceding
  final solution is qualified as}
$\{$\verb|(price,$100)|, \verb|(rating, null)|, \verb|(homepage,|
\verb| null)|$\}$,
\textit{but the latter solution is dropped because it is the same as the
  preceding final solution. The qualify-and-exclude-duplicate
  strategy is recursively applied to handle the nested OPTIONAL
  clauses. \\}

Also, we reduced the amount of writing of Section 6 merged Sections 5 and 6 of the original submissions. \\


\noindent \textbf{\large Reviewer 2 \\}

\noindent The second reviewer (R2) asked us to respond to specific revisions for D1 -- D3. \\

\noindent \textbf{R2.D1. I suggest that the authors further improve the experiment section by analyzing the effect of each optimization method separately. For instance, while the effect of optimization are overall impressive, -DEG and +REUSE does not show significant improvement in efficiency.\\}

Reflecting the reviewer's comment, to show the effect of each
optimization clearly, we measured the effect of each optimization
separately. The elapsed time reduced by each optimization is
illustrated in Figure~\ref{fig:effect-opt}, and the analysis of the
result is described in Section~\ref{sec:effect-five-optim} as follows. \\

\textit{Figure~\ref{fig:effect-opt} shows the reduced times of Q2 and
  Q9 in LUBM8000 after applying these optimizations separately.  The
  optimization techniques in X-axis are ordered by the reduced time in a
  decreasing manner --- \textsf{+INT}, \textsf{-NLF}, \textsf{-DEG},
  and \textsf{+REUSE}. Interestingly, even though Q2 and Q9 have the
  same shape (i.e., triangular), the most effective optimizations were
  different. \textsf{+INT} was the most effective in Q2. \textsf{-NLF}
  was the most effective in Q9 since the size of each candidate region
  was very small. \textsf{-DEG} was more effective in Q9 than in Q2
  since Q9 has more data vertices applied to the degree
  filter. \textsf{+REUSE} was effective in Q9 which has large number
  of candidate regions while Q2 did not benefit from
  \textsf{+REUSE}. \\}

Although neither -DEG nor +REUSE seems to show significant
improvement alone, these optimization techniques take effect after we
apply the other filters. That is, after applying +INT and -NLF, the
elapsed times for Q2 and Q9 were 701ms and 7257ms, respectively. Here, if
we further apply -DEG, the elapsed times became 297ms and 6049ms. This
shows that -DEG is indeed effective after applying the other filters. If
we then apply +REUSE, the elapsed times become 296ms and 5048ms. This shows
that +REUSE is effective in Q9. \\

\noindent \textbf{{R2.D2. Because many nodes in real-world graphs share a single type node (rdf:type), type-aware transformation may not decrease the size of most real-world graphs. The reviewer suggests presenting the graph size statistics for direct and type-aware transformation in the experiments.} \\}

To show the graph size reduction effect of the type-aware
transformation, we presented the graph size statistics of the direct
transformation and the type-aware transformation in
Table~\ref{tab:stat} and the description of such statistics as
follows. \\

\textit{Table~\ref{tab:stat} shows the number of vertices and edges of
  the graphs transformed by the direct transformation and the
  type-ware transformation. The reduced number of edges in the
  type-aware transformed graph directly affects the amount of graph
  exploration in e-graph homomorphism matching.}

\setcounter{table}{0}
\begin{table}[h!]
  \centering
	\resizebox{\linewidth}{!}{
  \begin{tabular}[h!]{|l|r|r|r|r|}
    \hline
    & $|V|$ direct & $|E|$ direct
    & $|V|$ type-aware & $|E|$ type-aware \\
    \hline
    LUBM80 & 2644579 & 19461754 & 2644573 & 12357312 \\
    LUBM800 & 26304872 & 193691328 & 26304863 & 122994224 \\
    LUBM8000 & 263133301 & 1937425416 & 263133295 & 1230263406 \\
    BTC2012 & 367728453 & 1436545556 & 367459811 & 1185887764 \\
    BSBM & 223938701 & 997822791 & 1937425416 & 893575906\\
    \hline
  \end{tabular}
	}
  \caption{Graph size statistics (direct: direct transformation, type-aware: type-aware transformation).}
  \label{tab:stat}
\end{table}

\noindent \textbf{{R2.D3. The authors may improve the
    presentation of the paper by adding citations/ explanation for
    some terms in the paper.} \\}

We have added full names of abbreviated terms and their citations
including NUMA, BSBM, LUBM, and BTC at their first occurrences. \\

\noindent \textbf{{R2.D4. Typos and grammatical errors}\\}

We have corrected all typos and grammatical errors. We appreciate your
thorough reviews. \\

\noindent \textbf{\large Reviewer 3 \\}

\noindent Thank you very much for your encouraging evaluation.
We detail our responses to your comments in the following section. \\

{\large \bfseries \noindent Additional comments from reviewers \\}

\noindent We also address the other comments from the reviewers. \\

\noindent \textbf{{R1.W1. The explanations of some experimental results
  must be further elaborated. For example, there is no way that one
  can see from Figure 7 that the recursive calls and/or IsJoinable are
  the dominating factors of poor performance.} \\}

Thank you for the valuable comment. We elaborated the explanation of the
experiment results in Figure~\ref{fig:comparison-direct-trans} using a
performance profiler, which had been excluded due to space limitations, as follows in
Section~\ref{sec:direct-transf}. \\

\textit{For long-running queries (i.e., Q2, Q6, Q9, and Q14),
  \TurboISOp{} is slower than some of its competitors. The performance of
	  \TurboISOp{} largely relies on 1) graph exploration by $ExploreCandidateRegion$ and 2) subgraph enumeration by $SubgraphSearch$. Moreover, when a query graph has
  non-tree edges, $IsJoinable$
  constitutes a large portion of $SubgraphSearch$. The profiling results of
  long running queries confirmed the above claims -- 1)
  $ExploreCandidateRegion$ and $SubgraphSearch$ are the dominating
  factors and 2) for queries which have non-tree edges (Q2 and Q9),
  $IsJoinable$ is the dominating factor of $SubgraphSearch$.
  Specifically, \TurboISOp{} spent the most time on
  $ExploreCandidateRegion$ (e.g. 46\% for Q2, 70\% for Q6, 72\% for
  Q9, and 69\% for Q14) and $SubgraphSearch$ (e.g. 54\% for Q2, 30\%
  for Q6, 28\% for Q9, and 31\% for Q14). Moreover, for queries which have
  non-tree edges, the most of $SubgraphSearch$ time was spent on
  $IsJoinable$ (e.g. 81.4\% for Q2 and 77.6\% for Q9).
 In order to speed up $ExploreCandidateRegion$, we propose a novel
  transformation (Section~\ref{sec:type-awre-transf}). Tailored optimization
  techniques are proposed for improving performance for both functions.
  (Section~\ref{sec:optimization}).\\}

% In addition, we further analyzed why $Q2$ benefited from the
% type-aware transformation did less than the other long running queries
% not, and had a significant elapsed time reduction with \textsf{+INT}
% in Section~\ref{sec:effect-type-aware}. \\

% \textit{Lastly, Q2 benefits less than the other long running queries
%   from the type-aware transformation. The following is the profiling
%   result of Q2 with the direct/type-aware transformation. Q2 with
%   direct transformation takes 26774.73 milliseconds in
%   $ExploreCandidateRegion$ and 31191.29 milliseconds in
%   $SubgraphSearch$.  Note that, with direct transformation, the
%   starting vertex is arbitrarily chosen from $u_0$, $u_1$, $u_2$ in
%   Figure~\ref{fig:direct-trans-query-graph-q2} since they all have
%   same vertex label frequency ($freq(g,L(u_i)) = 1, i = 0,1,2$) and
%   the same degree of $1$. In our implementation, the first query vertex
%   $u_0$ is chosen and thus the label of the non-tree edge is
%   \textsf{subOrganizationOf}. However, with type-aware transformation,
%   the starting vertex is $u_1$ in
%   Figure~\ref{fig:type-ware-trans-query-q2}, and the label of the
%   non-tree edge is \textsf{memberOf}. Although the number of candidate
%   regions with $u_1$ is the minimum among $u_0$, $u_1$, and $u_2$, the
%   cost of $IsJoinable$ calls for \textsf{memberOf} increases 1.30
%   times. Thus, Q2 with type-aware transformation takes 9523.60
%   milliseconds in $ExploreCandiateRegion$ and 40469.47 milliseconds in
%   $SubgraphSearch$. We achieve only 1.16 times performance
%   improvement. However, the cost of the $IsJoinable$ call is significantly
%   reduced by using \textsf{+INT}. Thus, after applying type-aware
%   transformation and the tailored optimizations, the final elapsed
%   time for Q2 becomes 309.74ms, i.e., 187.15 times performance
%   improvement compared with direct transformation only. \\}

\noindent \textbf{{R2.D4. Some drawbacks of type-aware
    transformation are update/ deletion anomalies, in particular, when
    the graph has a long chain of types (using rdf:subClassOf).  By
    any change in the chain, the data structure of all of the
    instances of corresponding types should be update.} \\ }

We appreciate your valuable comment, the topic of which will be our next research
direction. In the paper, we assumed periodic batch updates of a
graph. We have referred to this as our future work in
Section~\ref{sec:data-structure} as
follows. \\

\textit{We assume that graphs in our system are periodically updated from an underlying RDF source. For efficient graph update, a
  transactional graph store is definitely required. We leave this
  exploration to future work since it is beyond the scope of the
  paper.\\}

\noindent \textbf{{R3.D1. The paper indicates that graph isomorphism
  algorithms can be easily modified to deal with graph homomorphism,
  but the issue is not addressed further. Some justification for this
  claim would be helpful.} \\}

We have provided the detailed discussion in Section~\ref{sec:turbo_iso} on how subgraph isomorphism algorithms
can be easily modified to handle graph homomorphism as follows. \\

	\textit{ We first explain how the generic subgraph isomorphism algorithm \cite{LHK:12aa} can easily handle graph homomorphism. The generic subgraph isomorphism algorithm is implemented as a
backtrack algorithm, where we find solutions by incrementing
partial solutions or abandoning them when it is determined that they cannot be
completed. Here, given a query graph $q$ and its matching order ($u_{\sigma(1)}$, $u_{\sigma(2)}$, ..., $u_{\sigma(|V(q)|)}$),
a solution is modeled as a vector $\vec{v}$ = ($M({u_{\sigma(1)}})$, $M({u_{\sigma(2)}})$, ..., $M({u_{\sigma(|V(q)|)}})$) where
each element in $\vec{v}$ is a data vertex for the corresponding query vertex in the matching order.
At each step in the backtrack algorithm, if a partial solution is given,
we extend it by adding every possible candidate data vertex at the end.
Here, any candidate data vertex that does not satisfy the following three
conditions must be pruned.  }
 \begin{enumerate}[1)]
\item $\forall u_i \in V(q)$, $L(u_i) \subseteq L(M(u_i))$
\item $\forall (u_i, u_j) \in E(q)$, $(M(u_{i}), M(u_{j})) \in E(g)$ and $L(u_{i}, u_{j}) = L(M(u_{i}), M(u_{j}))$
\item $M(u_i) \neq M(u_j)$ if $u_i \neq u_j$
\end{enumerate}

\textit{
Note that the third condition ensures the injective condition, guaranteeing
that no duplicate data vertex exists in each solution vector.
Thus, by just disabling the third condition, the generic subgraph
isomorphism algorithm finds all possible homomorphisms.
}
\textit{
Now, we describe how to disable the third condition in \TurboISO{}, which
is an instance of the generic subgraph isomorphism algorithm.
\TurboISO{} uses pruning rules by applying filters in both
$Explore\-CandidateRegion$ and $SubgraphSearch$. First, the degree filter and the NLF filter should be modified since a data vertex can be mapped to
multiple query vertices. The degree filter qualifies data vertices
which have an equal number or more neighbors than distinct labels of
their corresponding query vertices. The NLF filter qualifies data
vertices which have at least one neighbor for all distinct labels of
their corresponding query vertices.
Second, lines 4--6 of $SubgraphSearch$ ensuring the third condition should be removed in
order to disable the injectivity test. As we see here, with minimal
modification to \TurboISO{}, it can easily support graph homomorphism.
}
\textit{
In order to make \TurboISO{} handle the e-graph homomorphism, the query
edge to edge label mapping, $M_e$, should be additionally added in
$SubgraphSearch$.
For this, $UpdateState$ assigns $M_e(P(q',u), u)$ = $L(M_v(P(q',u)), M_v(u))$
, and $RestoreState$ removes such mapping.
From here on, let us denote
\TurboISO{} modified for the e-graph homomorphism as \TurboISOp{}.\\
}

\noindent \textbf{{R3.D2. Graph homomorphism algorithms are applied to
  RDF graphs after the RDF graph is converted to a property
  graph. This is stated, but not developed. I would address (a) why
  this is necessary and why homomorphism algorithms cannot be made to
  work on RDF graphs directly, and (b) how feasible this conversion is
  in general.} \\}

Thank you for pointing this out to us. We addressed the e-graph
homomorphism on the type-aware transformed graph as follows in
Section~\ref{sec:type-awre-transf}.

\textit{Now, we explain how the generic e-graph homomorphism
  algorithm works for type-aware transformed query/data graphs.
  When appending a candidate data vertex to the current partial
  solution, we additionally check the following condition for the ID
  attribute of the two-attribute vertex model.
}
  \[ \forall u \in \{u | ID(u) \neq \_ \text{ for } u \in V \}, ID(u)
  = ID'(M_v(u)).\]

As stated in Section~\ref{sec:preliminary}, the graph homomorphism
should consider additional edge mapping to apply RDF query
processing. The resulting e-graph homomorphism algorithm is
\TurboISOp{}, which is directly applicable to RDF graphs. However, to
improve efficiency, we proposed \TurboISOP{} which improves
performance using type-aware transformation and tailored optimization
techniques. Also, Definition~\ref{def:type-aware} defines a general
conversion from an RDF graph to a type-aware transformed graph (a special
		case of the property graph). \\

\noindent \textbf{{R3.D3. The approach is not sound under the
    simple entailment regime, as far as I know. This is easy to fix.}
  \\}

Thank you for the valuable comment. In the paper, to get a correct
solution for LUBM queries, we assumed an entailment regime which can
infer triples having \textsf{rdf:type} predicate from triples having
\textsf{rdf:subClassOf} predicate (e.g. RDFS entailment regime).

One way to deal with the simple entailment regime in the type-aware
transformed graph is to distinguish
$L_{simple}(v) = \{F_{L_V}(o) | \text{there is an edge from }
F_V^{-1}(v) \text{ to } o \text{ using triples in } T'\}$
from $L(v)$. \TurboISOP{} can process a SPARQL query under the simple
entailment regime using $L_{simple}(v)$ instead of $L(v)$.  We briefly
mentioned
this in Section~\ref{sec:data-structure} as follows. \\

\textit{Note also that \TurboISOP{} can also handle SPARQL queries
  under the simple entailment regime correctly. In order to deal with
  the simple entailment regime in the type-aware transformed graph,
  \TurboISOP{} distinguishes
  $L_{simple}(v) = \{F_{L_V}(o) | \text{there is an edge from }
  F_V^{-1}(v) \text{ to } o \text{ using triples in } T'\}$
  from $L(v)$. \TurboISOP{} can process a SPARQL query under the
  simple entailment regime using $L_{simple}(v)$ instead of
  $L(v)$. \\}

\noindent \textbf{Minor comments from R1.}

In the first paragraph of Section~\ref{sec:rdf-as-graph}, we changed
the term ``certain relationships'' to ``type relationships'' according
to your suggestion.

In notation, we used the subscripts and the superscripts
consistently. For example, subscript $i$ is consistently used for a
node index.

		 \iffalse

\noindent \textbf{{R1.D1. Can the paper and its experiment
    provide more evidences to illustrate the main research problem and
    they are solved by any specific proposed techniques?} \\}

As we mentioned in R1.W1, The dominating factors of \TurboISOp{} are
$ExploreCandidateRegion$ and $SubgraphSearch$ in which $IsJoinable$ is
dominant. Accordingly, our research problem addresses both dominating
factors by proposing the type-ware transformation and tailored
optimization techniques --- \edit{1) the type-aware transformation,
\textsf{-NLF}, and \textsf{-DEG} for $ExploreCandidateRegion$, and 2)
\textsf{+INT} for $IsJoinable$ and
\textsf{+REUSE} for $DetermineMatchingOrder$.} \\


In Section~\ref{sec:introduction}, we briefly mentioned both
dominating
factors as follows: \\
\textit{By transforming RDF graphs into labeled graphs, we can apply
  subgraph homomorphism methods to RDF query processing. Extensive
  experiments using several benchmarks show that naive modification of
  \TurboISO{} outperforms the RDF processing engines for queries which
  require a small amount of graph exploration. However, for some
  queries which require a large amount of graph exploration, the naive
  modification is slower than some of its competitors. Two dominant
  parts of \TurboISO{} --- 1) exploring candidate subgraphs and 2)
  searching subgraphs based on candidate subgraphs --- give a room for
  improvement. \TurboISOP{} resolves such performance hurdles by
  proposing \emph{the type-aware transformation} and tailored
  optimization techniques. \\}

In the last paragraph of Section~\ref{sec:direct-transf}: \\
\textit{... To improve the efficiency on those dominating factors, we
  further optimize the e-graph homomorphism algorithm
  (e.g. \TurboISOp{}) by a novel transformation and tailored
  optimization techniques (Section~\ref{sec:turbohom++}). \\}

In Section~\ref{sec:optimization}, we reordered optimization
techniques in a decreasing order of their effect --- \textsf{+INT},
\textsf{-NLF}, \textsf{-DEG}, and \textsf{+REUSE}. Also, we specified
where \textsf{-NLF} and \textsf{-DEG} are used. \\

	  \fi
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "turbordf.pvldb"
%%% End:


==> typeaware-transform.tex <==
\section{RDF Query  Processing by \edit{Graph Homomorphism}}
\label{sec:sparql-proc-subgr}

In this section, we discuss how RDF datasets can be naturally viewed
as graphs (Section~\ref{sec:rdf-as-graph}), and thus how an RDF
dataset can be directly transformed into a corresponding labeled graph
(Section~\ref{sec:direct-transf}). After such a transformation,
henceforth, \edit{the subgraph isomorphism algorithms modified for the
  graph homomorphism such as \TurboISOp{}} can be applied for
processing SPARQL queries.

For the sake of optimizing query performance, however, we propose a
novel method of transforming RDF data into labeled graph, namely
\textit{type-aware transformation}
(Section~\ref{sec:type-awre-transf}). Our type-aware transformation
embeds the \verb|rdf:type| of a subject into the subject's attribute
and thus creates a smaller query graph than direct transformation.

\subsection{RDF as Graph}
\label{sec:rdf-as-graph}

An RDF dataset is a collection of triples each of which consists of a
subject, a predicate, and an object. 
% The purpose of RDF is to describe resources or concepts, and to model information \cite{LSW:98aa}. 
Figure~\ref{fig:rdf} is an example RDF dataset that
captures certain relationships between university organizations
and students.

\begin{figure}[h!]
  \centering
   \scriptsize
   \begin{tabular}{lll}
      $\langle$subject$\rangle$ & $\langle$predicate$\rangle$ & $\langle$object$\rangle$ \\
      student1 & rdf:type  & GraduateStudent \\
      GraduateStudent & rdf:subClassOf & Student \\
      univ1 & rdf:type & University \\
      dept1.univ1 & rdf:type & Department \\
      student1 & undergradDegreeFrom & univ1 \\
      student1 & memberOf & dept1.univ1 \\
      dept1.univ1 & subOrganizationOf & univ \\
      student1 & emailAddress & `john@dept1.univ1.edu' \\
      student1 & telephone & `012-345-6789' \\
   \end{tabular}
  \caption{RDF triples.}
  \label{fig:rdf}
\end{figure}

By considering triples as directed edges, an RDF dataset naturally
becomes a directed graph: the subjects and the objects are
vertices while the predicates are edges. Figure~\ref{fig:graph} is the
graph representation of triples in Figure~\ref{fig:rdf}. Note that we use
rectangles to represent vertices in RDF graphs to distinguish
them from the labeled graphs.

\begin{figure}[h!]
  \centering
  \includegraphics[width=1\linewidth]{graph}
  \caption{RDF graph.}
  \label{fig:graph}
\end{figure}

\subsection{Direct Transformation}
\label{sec:direct-transf}

In order to apply conventional subgraph isomorphism algorithms
modified \edit{for graph homomorphism (e.g. \TurboISOp{})} to RDF query
processing, RDF graphs has to be transformed into labeled graphs
first.

The most basic way to transform RDF graphs is (1) to map subjects and
objects to vertex IDs and (2) to map predicates to edge labels. We
call such transformation as the \textit{direct transformation} because
the topology of the RDF graph is kept in the labeled graph after the
transformation. Figure~\ref{fig:direct-transformation} shows the
result of the direct transformation of the example RDF graph of
Figure~\ref{fig:graph} -- Figures~\ref{fig:direct-sub-obj-map},
\ref{fig:direct-pred-map}, and~\ref{fig:direct-trans-graph} are the
vertex ID mapping table, the edge label mapping table, and the
transformed graph, respectively.

\setlength{\tabcolsep}{0.5mm}
\begin{figure}[h!]
  \centering
  \subfloat[vertex label mapping table.]
  {
    \label{fig:direct-sub-obj-map}
    \scriptsize
    \begin{tabular}[t]{|c|c|}
      \hline
      Subject/Object & VertexID \\
	  \hline
	  GraduateStudent & $v_0$ \\
	  Student & $v_1$ \\
	  University & $v_2$ \\
	  Department & $v_3$ \\
	  student1 & $v_4$ \\
	  univ1 & $v_5$ \\
	  dept1.univ1 & $v_6$ \\
	  `john@dept1.univ1.edu'& $v_7$ \\
	  `012-345-6789'& $v_8$ \\
      \hline
    \end{tabular}
  }
  \subfloat[edge label mapping table.]
  {
    \label{fig:direct-pred-map}
    \scriptsize
    \begin{tabular}[t]{|c|c|}
      \hline
      Predicate & Edge Label \\
      \hline
       rdf:type & a  \\
       rdf:subClassOf & b  \\
       undergradDegreeFrom & c \\
       memberOf & d \\
       subOrganizationOf & e \\
       telephone & f \\
       emailAddress & g \\
      \hline
    \end{tabular}
  }
  \\
  \subfloat[graph.]
  {
    \label{fig:direct-trans-graph}
    \includegraphics[width=0.6\linewidth]{direct-transformation}
  }
  \caption{Direct transformation of RDF graph.}
  \label{fig:direct-transformation}
\end{figure}

Unlikely to a data graph, a query graph is obtained from a SPARQL query. A
query vertex may hold the data vertex ID which corresponds to the subject or
object specified in the SPARQL query. If the query vertex corresponds to a
variable, the data vertex is left as blank.  For example, the SPARQL query of
Figure~\ref{fig:direct-trans-sparql-q2} is transformed into the query graph of
Figure~\ref{fig:direct-trans-query-graph-q2}.  Here the query vertex $u_0$,
which corresponds to \verb|Student|, holds the data vertex ID $v_1$; To the
contrary, the query vertex $u_3$, which corresponds to the variable $X$, has
blank (\verb|_|) as the data vertex ID.  Similarly, a query edge may hold the
edge label which corresponds to the predicate. For example, the edge label of
$(u_3, u_4)$ is $c$ as the edge corresponds to the \verb|undergradDegreeFrom|
predicate. 

\begin{figure}[h!]
  \centering

  \begin{myverbbox}{\vqtwo}
SELECT ?X, ?Y, ?Z WHERE
{?X rdf:type Student .
 ?Y rdf:type University .
 ?Z rdf:type Department .
 ?X undergradDegreeFrom ?Y .
 ?X memberOf ?Z .
 ?Z subOrganizationOf ?Y.}
    \end{myverbbox}
  \subfloat[SPARQL query.]
  {
    \label{fig:direct-trans-sparql-q2}
    \resizebox{0.5\linewidth}{!}{ \raisebox{5mm}{\vqtwo}}
  }
  \subfloat[query graph.]
  {
    \label{fig:direct-trans-query-graph-q2}
    \includegraphics[width=0.5\linewidth]{direct-transformation-q2}
  }
  \caption{Direct transformation of SPARQL query.}
  \label{fig:direct-transformation-query}
\end{figure}

\edit{Note that, when a variable is declared on a predicate in a
  SPARQL query, a graph homomorphism algorithm can answer such SPARQL
  query by having an additional mapping from query edges, which
  correspond to variables on predicates, to their corresponding edge
  labels in a data graph. This edge label mapping can be done in
  $UpdateState$. We will see such queries which has variables on
  predicates in Section~\ref{sec:experiment}. }

Consequently, the direct transformation makes it possible to apply
conventional \edit{graph homomorphism} algorithms for processing SPARQL
queries on RDF datasets. In order to evaluate the performance of such
an approach, we applied \edit{\TurboISOp{}}, the state-of-the-art
subgraph isomorphism algorithm \edit{which is modified for graph
  homomorphism}, on LUBM8000, a billion-triple RDF benchmark, after
applying direct transformation. We compared the performance of
\edit{\TurboISOp{}} against two existing RDF engines: RDF-3X
\cite{NW:10aa}, and System-X\footnote{We anonymize the product name to
  avoid any conflict of interest.}.
Figure~\ref{fig:comparison-direct-trans} depicts the measured
execution time of these three systems in log scale. (See
Section~\ref{sec:experiment-setup} for the details of the experiment
setup)

To our surprise, although there is no clear winner among them, the
figure reveals that \edit{\TurboISOp{}} already performs as good as
the existing RDF engines. For those long-running queries (i.e., Q2,
Q6, Q9, Q14), \edit{\TurboISOp{}} is slower than some of its
competitors. This poses an important research question to us,
``\emph{Is this phenomenon due to inherent limitation of the subgraph
  isomorphism algorithm?}'' In order to address this problem, we
propose (1) \textit{type-aware transformation}
(Section~\ref{sec:type-awre-transf}) and (2) a series of optimizations
(Section~\ref{sec:optimization}).

\begin{figure}[h!]
  \centering
  \includegraphics[width=\linewidth]{comparison-direct-trans}
  \caption{Comparison between original \TurboISOp{} with the direct
    transformation graph and other RDF engines.}
  \label{fig:comparison-direct-trans}
\end{figure}

\subsection{Type-aware Transformation}
\label{sec:type-awre-transf}

In this subsection, we propose another method for transforming an RDF
graph into a labeled graph which can result in faster pattern matching
than direct transformation. To enable this new transformation, we
first devise the \textit{two-attribute vertex model} which makes use
of the type information specified by the \verb|rdf:type| predicate.
Specifically, this model assumes that each vertex is associated with a
set of labels (the label attribute) in addition to its ID (the ID
attribute). The label attribute is obtained by following the predicate
\verb|rdf:type| -- if a subject has one or more \verb|rdf:type|
predicates, its types can be obtained by following the \verb|rdf:type|
(as well as \verb|rdf:subClassOf| predicates transitively) while
collecting corresponding objects. For example, \verb|student1| in
Figure~\ref{fig:graph} has the label attribute,
$\{\verb|GradStudent|,$ $\verb|Student|\}$.

The above two-attribute vertex model naturally leads to our new RDF
graph transformation, \textit{the type-aware transformation}. Here,
subjects and objects are transformed to two-attribute vertices by
utilizing \verb|rdf:type| predicates as described above. Then, the ID
attribute corresponds to the vertex ID, and the label attribute
corresponds to the vertex label. An additional vertex label mapping
table is generated accordingly.
Figure~\ref{fig:type-aware-transformation} shows an example of the
mapping tables and the data graph, which is the result of applying
type-aware transformation to the RDF graph of Figure~\ref{fig:graph}.

Note that objects having only \verb|rdf:type| and
\verb|rdf:subClassOf| are not transformed into data graph vertices at
all since these are simply type information which is already embedded
as the label attribute of some other vertices. For example, objects
like \verb|GradStudent|, \verb|Student|, \verb|University|, and
\verb|Department| in Figure~\ref{fig:graph} do not create any vertex
in Figure~\ref{fig:type-aware-trans-graph}. Similarly, the predicates
\verb|rdf:type| and \verb|rdf:subClassOf| do not create any edge after
type-aware transformation.

\setlength{\tabcolsep}{0.7mm}
\begin{figure}[h!]
  \centering
  \subfloat[vertex ID mapping table.]
  {
    \label{fig:type-aware-vid-map}
    \scriptsize
    \begin{tabular}[t]{|c|c|}
      \hline
      Subject/Object & Vertex ID \\
	  \hline
	  student1 & $v_0$ \\
	  univ1 & $v_1$ \\
	  dept1.univ1 & $v_2$ \\
	  `john@dept1.univ1.edu' & $v_3$ \\
	  `012-345-678' & $v_4$ \\   
      \hline
    \end{tabular}
  }
  \hspace*{0.15cm}
  \subfloat[vertex label mapping table.]
  {
    \label{fig:type-aware-vlabel-map}
    \scriptsize
    \begin{tabular}[t]{|c|c|}
      \hline
      Vertex label & type \\
      \hline
      A & GraduateStudent \\
      B & Student \\
      C & University \\
      D & Department \\
      \hline
    \end{tabular}
  }
  \\
  \subfloat[edge label mapping table.]
  {
    \label{fig:type-aware-elabel-map}
    \scriptsize
    \begin{tabular}[b]{|c|c|}
      \hline
      Edge label & Predicate \\
      \hline
      a & undergradDegreeFrom \\
      b & memberOf \\
      c & subOrganizationOf \\
      d & telephone \\
      e & emailAddress \\
      \hline
    \end{tabular}
  }
  \subfloat[data graph.]
  {
    \label{fig:type-aware-trans-graph}
    \includegraphics[width=0.4\linewidth]{type-aware-transformation}
  }
  \caption{Type-aware transformation of an RDF graph.}
  \label{fig:type-aware-transformation}
\end{figure}

Likewise, a SPARQL query is transformed into the corresponding query
graph. As an example, Figure~\ref{fig:type-ware-trans-query-q2} is the
query graph type-aware transformed from the SPARQL query in
Figure~\ref{fig:direct-trans-sparql-q2}. Note that, as in the case of
direct transformation, we use blank (\_) if no vertex label (or data
vertex ID) is specified in a transformed query graph.

\begin{figure}[h!]
  \centering
  \includegraphics[width=0.35\linewidth]{type-aware-transformation-q2}
  \caption{Type-aware transformation of SPARQL query
    of Figure~\ref{fig:direct-trans-sparql-q2}.}
  \label{fig:type-ware-trans-query-q2}
\end{figure}

The virtue of the type-aware transformation is that it can improve the
efficiency of RDF query processing. Since the type-aware
transformation eliminates certain vertices and edges by embedding {\it
  type} information into the vertex label, the resulting query graph
has a smaller size and simpler topology than direct transformation.

As an example, let us consider the SPARQL query in
Figure~\ref{fig:direct-trans-sparql-q2}. After direct transformation,
it becomes the query graph in
Figure~\ref{fig:direct-trans-query-graph-q2} that has a relatively
complex topology consisting of six vertices and six edges. On the
other hand, the type-aware transformation produces the query graph in
Figure~\ref{fig:type-ware-trans-query-q2} that has a simple triangle
topology. This reduced number of vertices and edges has a positive
effect on efficiency because it results in less graph exploration.

% In addition, the simplified topology from type-aware transformation
% also contributes significantly to increasing the efficiency.
% For instance, the query graph in
% Figure~\ref{fig:type-aware-trans-sparql-q8} has simple path topology
% (as opposed to more complicated tree topology that direct transformation
% would produce for the same query) --
% \TurboISO{} can answer this query very quickly since it can
% omit several time-consuming steps for such simple topology.

% \begin{figure}[h!]
%   \centering
%   \begin{myverbbox}{\vqeight}
% SELECT ?X, ?Y, ?Z WHERE
% {?X rdf:type Student .
%  ?Y rdf:type Department .
%  ?X ub:memberOf ?Y .
%  ?Y ub:subOrganizationOf univ1 .
%  ?X ub:emailAddress ?Z}
%   \end{myverbbox}
%   \subfloat[SPARQL query.]
%   {
%     \label{fig:type-aware-trans-sparql-q8}
%     \vqeight
%   }
%   \subfloat[query graph.]
%   {
%     \label{fig:type-aware-trans-query-graph-q8}
%     \includegraphics[width=0.35\linewidth]{type-aware-trans-q8}
%   }
%   \caption{Another type-ware query transformation example.}
%   \label{fig:type-aware-trans-query-q8}
% \end{figure}

\subsection{Data Structures}
\label{sec:data-structure}

\TurboISOp{} maintains two in-memory data structures for the data graph
to support efficient graph exploration. The inverse vertex label list
supports the efficient retrieval of data vertex IDs for a given vertex
label. It contributes to the efficient processing on (1) computing the
ranking score in \edit{selecting a starting query vertex} and (2)
collecting the starting data vertices.
% $v_s$ in line 3 of Algorithm~\ref{alg:turboiso}.
Figure~\ref{fig:inverse-vertex-list}
shows the inverse vertex label list of
Figure~\ref{fig:type-aware-trans-graph}. The `end offsets' records the
exclusive end offset of the `vertex IDs' for each vertex label.

The adjacency list supports efficient retrieval of the adjacent data
vertices for the given vertex, edge label, and vertex label. It
contributes to the efficient processing in \edit{candidate region
  exploration} %$ExploreCandidateRegion$
and \edit{$IsJoinable$}. Figure~\ref{fig:adjacency-list} shows the
adjacency list of Figure~\ref{fig:type-aware-trans-graph} for the
outgoing edges. The adjacency list stores the adjacent vertices for
each data vertex in the same way as the inverse vertex label list. One
difference is that the adjacency list has an additional array (`end
offsets') to group the adjacent vertices of a data vertex for each
neighbor type. Here, the neighbor type refers to the pair of the edge
label and the vertex label. For example, $v_0$ in
Figure~\ref{fig:type-aware-trans-graph}, has four different neighbor
types -- $(a,C), (b,D), (d,\_)$ and $(e,\_)$. Those four neighbor
types are stored in `end offsets,' and each entry points to the
exclusive end offset of the `adjacent vertex ID'. Note that
\TurboISOp{} maintains another adjacency list for the incoming edges.

\begin{figure}[h!]
  \centering
  \subfloat[inverse label vertex list.]
  {
    \label{fig:inverse-vertex-list}
    \includegraphics[width=0.43\linewidth]{inverse-vertex-list}
  }
  \\
  \subfloat[adjacency list.]
  {
    \label{fig:adjacency-list}
    \includegraphics[width=0.9\linewidth]{adjacency-list}
  }
  \caption{In-memory data structures for the data graph of
    Figure~\ref{fig:type-aware-trans-graph} ($adj(v):$ adjacent
    vertices of $v$, $adj(v,(el,vl)):$ adjacent vertices $v$, which
    have vertex label $vl$ and are connected with edge label $el$).}
  \label{fig:datastructure}
\end{figure}

If the starting query vertex specifies the vertex label, the
corresponding data vertices are retrieved using the inverse vertex
list. Otherwise, the data vertex ID specified in the starting query
vertex is used. Once the starting data vertices are identified, the
candidate region exploration continues by exploiting the adjacency
information stored in the adjacency list. \edit{In case that a
  complete adjacency information is not given, \TurboISOp{} finds the
  correct adjacent vertices by 1) collecting all adjacent vertices
  which match the incomplete information and 2) removing duplicated
  vertices.}

We extend \TurboISOp{} so that it can handle SPARQL queries where a
query vertex has no label or \text{ID} at all. In order to handle such
queries, we maintain an index called the predicate index where a key
is a predicate, and a value is a pair of a list of subject IDs and a
list of object IDs. This index is used 1) to compute the cardinality
of a query vertex $u$ in $Choose\-Start\-Query\-Vertex$ when $u$ has
no label and 2) to find candidate data vertices for the starting query
vertex having no label.

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "turbordf.pvldb"
%%% End:

